False Discovery Rate Control via Prediction-Based, Model-Agnostic Data Splitting: An Application to Gut Microbiome Data in Liver Function

Many methods have been proposed to control the false discovery rate (FDR) in feature selection, yet challenges remain when the relationship between predictors and the outcome is complex. We propose a prediction-based data-splitting procedure that can leverage flexible predictive models while controlling the FDR. The data are divided into three parts: one for model training and two for constructing the mirror statistic. For each feature, we construct a negative control using the remaining features without incorporating outcome information and define a test statistic based on the resulting change in predictive performance. Under the null, such a perturbation is approximately equally likely to increase or decrease predictive performance, yielding a statistic symmetric about zero. In contrast, perturbing an informative feature tends to reduce predictive performance, resulting in a large positive statistic. Features are selected by thresholding these statistics, with false discoveries estimated from the corresponding negative tail to control the FDR. We apply the proposed method to liver function microbiome data, where high-dimensional, correlated features and potentially complex feature--outcome relationships make reliable type I error control particularly important for reproducible scientific discovery. Through simulation studies and the real-data application, we demonstrate that the proposed framework provides robust FDR control and can be integrated with state-of-the-art machine-learning models to accommodate complex relationships between features and the outcome.

==> logRatioInput.tex <==
\section{Discussion about log ratio transformation as the input for predictive models}

Although log-ratio transformations provide an effective framework for addressing
the compositional nature of microbiome data, we do not use log-relative
abundances as the primary input for predictive models in this work. The reason
is that the scientific objective of this study is not only to achieve accurate
prediction, but also to identify individual microbial features that contribute
to the prediction. A log-ratio transformation fundamentally changes the unit of
analysis from individual features to relative contrasts between features. For
example, the centered log-ratio transformation is defined as
\[
\mathrm{clr}(x_j)=\log(x_j)-\frac{1}{p}\sum_{k=1}^{p}\log(x_k),
\]
where the transformed value of feature $j$ depends not only on its own
abundance but also on the abundance of all other features. Consequently, a
predictive signal attributed to a transformed feature may reflect a change in
the focal taxon, changes in other taxa included in the geometric mean, or a
combination of both. While such relative representations are highly useful for
inference on compositional contrasts, they make direct attribution of predictive
importance to individual microbial features less straightforward. Because our
primary goal is feature-level discovery through perturbation-based predictive
importance measures, we retain the original abundance scale as the input to the
predictive models and separately evaluate whether enforcing compositional
constraints in the negative-control construction affects the results.


